SP-BatikGAN: An Efficient Generative Adversarial Network for Symmetric Pattern Generation

Following the contention of AI arts, our research focuses on bringing AI for all, particularly for artists, to create AI arts with limited data and settings. We are interested in geometrically symmetric pattern generation, which appears on many artworks such as Portuguese, Moroccan tiles, and Batik, a cultural heritage in Southeast Asia. Symmetric pattern generation is a complex problem, with prior research creating too-specific models for certain patterns only. We provide publicly, the first-ever 1,216 high-quality symmetric patterns straight from design files for this task. We then formulate symmetric pattern enforcement (SPE) loss to leverage underlying symmetric-based structures that exist on current image distributions. Our SPE improves and accelerates training on any GAN configuration, and, with efficient attention, SP-BatikGAN compared to FastGAN, the state-of-the-art GAN for limited setting, improves the FID score from 110.11 to 90.76, an 18% decrease, and model diversity recall score from 0.047 to 0.204, a 334% increase.

==> content/6.future-work.tex <==
\label{section:future}
The author highly recommends the use of density in future research, which in essence, is a much more informative precision. With density, we can thoroughly analyze Generator behavior.

Interestingly, while StyleGAN2 with SAN is able to improve significantly \cite{yu2021dual}, however for limited computation using FastGAN further research needed to be done to implement attention. Even with EAttention SP-BatikGAN need SPE loss to accelerate training.

For Batik generation, while this research only focuses on the squared symmetrical pattern type, we believe the flexibility of different SPE symmetric operations is also the key and can be used on other different batik types. For example is Batik Parang, which is a batik with a diagonal repeating seamless pattern. Future research is also needed for many different complex types of patterns.

While we succeed in training a high-quality GAN, for further meaningful application, the ability to control the latent space and find a meaningful vector to control image output will be the future of this applied research. Such an example is to use the well-known GAN Space control \cite{2020ganspace} to extrapolate meaningful latent.

For future research we are currently applying our Seamless Pattern Enforcement into a diffusion based model.
